Online Guest Detection in a Smart Home using Pervasive Sensors and Probabilistic Reasoning

Smart home environments equipped with distributed sensor networks are capable of helping people by providing services related to health, emergency detection or daily routine management. A backbone to these systems relies often on the system's ability to track and detect activities performed by the users in their home. Despite the continuous progress in the area of activity recognition in smart homes, many systems make a strong underlying assumption that the number of occupants in the home at any given moment of time is always known. Estimating the number of persons in a Smart Home at each time step remains a challenge nowadays. Indeed, unlike most (crowd) counting solution which are based on computer vision techniques, the sensors considered in a Smart Home are often very simple and do not offer individually a good overview of the situation. The data gathered needs therefore to be fused in order to infer useful information. This paper aims at addressing this challenge and presents a probabilistic approach able to estimate the number of persons in the environment at each time step. This approach works in two steps: first, an estimate of the number of persons present in the environment is done using a Constraint Satisfaction Problem solver, based on the topology of the sensor network and the sensor activation pattern at this time point. Then, a Hidden Markov Model refines this estimate by considering the uncertainty related to the sensors. Using both simulated and real data, our method has been tested and validated on two smart homes of different sizes and configuration and demonstrates the ability to accurately estimate the number of inhabitants.

==> sections/introduction-SotA.tex <==
Ambient Assisted Living (AAL) systems are systems that aim at empowering people capabilities using Ambient Intelligence, meaning digital pervasive environments capable of reacting and adapting to their users' need. AAL technologies provide services such as health control, emergency detection systems or activity monitoring. (REFS) Recent advancement in various technological areas such as pervasive sensing, robotics and human-machine interaction brings these systems closer and closer to becoming a reality for everyone. However, most existing projects and research still fail to overcome one particular problem: the possibility of having an unknown number of persons in the environment. Indeed, such systems usually use techniques that have been designed or trained for one (sometimes two) occupants and cannot tackle other numbers of persons. However, real-life situations usually involve visits from other persons, especially in the domain of AAL where the users considered are often persons living alone or with their partner, and are regularly visited by caregivers. So far, the most common strategy is to stop the system or annotate when more persons than expected are present in the environment in order to avoid incorrect inferences. (REF REF REFs!). 

Being able to detect if a person is alone or not, and to a certain extend count the number of persons in the environment is of great importance for the development of AAL systems. This paper aims at tackling this specific problem by proposing a framework combining a Constraint Satisfaction Problem Solver with a Hidden Markov Model in order to estimate the number of persons present in an environment. Our system has been evaluated on simulated and real data 

\section{Related work}
1* about person counting
2* about integrating CSP and probabilistic reasoning
